Meritocracy and Its Discontents: Long-run Effects of Repeated School Admission Reforms

What happens if selective colleges change their admission policies? We study this question by analyzing the world's first implementation of nationally centralized meritocratic admissions in the early twentieth century. We find a persistent meritocracy-equity tradeoff. Compared to the decentralized system, the centralized system admitted more high-achievers and produced more occupational elites (such as top income earners) decades later in the labor market. This gain came at a distributional cost, however. Meritocratic centralization also increased the number of urban-born elites relative to rural-born ones, undermining equal access to higher education and career advancement.

==> exhibits/adm_taxsample_gap.tex <==
\begin{tabular}{lcccc}
\toprule
\toprule
                    &\multicolumn{4}{c}{Sampling rate of PIR relative to tax record}\\\cmidrule(lr){2-5}
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{\shortstack{Top 0.01\%\\PIR (1934)}}&\multicolumn{1}{c}{\shortstack{Top 0.01\%\\PIR (1939)}}&\multicolumn{1}{c}{\shortstack{Top 0.05\%\\PIR (1939)}}&\multicolumn{1}{c}{\shortstack{Top 0.05\%\\PIR (1934)}}\\
\hline  \\ 
Entrants to Schools 1--8 per birth population&    -0.00176   &    -0.00157   &     0.00098   &    -0.00083   \\
                    &     (0.425)   &     (0.667)   &     (0.540)   &     (0.499)   \\
Observations        &          47   &          47   &          47   &          47   \\
Mean dep var        &     0.42990   &     0.60362   &     0.19342   &     0.32783   \\
\hline \hline
\end{tabular}


==> exhibits/jpir_total_nobs.tex <==
\begin{tabular}{lcc} \hline \hline
 & (1) & (2) \\
 & \multicolumn{2}{c}{No. of Individuals in PIR} \\ 
 & \multicolumn{2}{c}{(No. of individuals aged 50 in PIR = 100)} \\ \hline
 &  &  \\
Age 17 under centralization & 3.77 &  \\
 & (0.086)* &  \\
 Cohort's exposure to centralization &  & 4.78 \\
 &  & (0.060)* \\
Age & 40.32 & 39.69 \\
 & (0.000)*** & (0.000)*** \\
Age squared & -0.39 & -0.38 \\
 & (0.000)*** & (0.000)*** \\
PIR (1939) dummy & 0.37 & 0.37 \\
 & (0.808) & (0.805) \\
 &  &  \\
Observations & 46 & 46 \\ \hline \hline
\end{tabular}
